Consistent Text Categorization using Data Augmentation in e-Commerce

The categorization of massive e-Commerce data is a crucial, well-studied task, which is prevalent in industrial settings. In this work, we aim to improve an existing product categorization model that is already in use by a major web company, serving multiple applications. At its core, the product categorization model is a text classification model that takes a product title as an input and outputs the most suitable category out of thousands of available candidates. Upon a closer inspection, we found inconsistencies in the labeling of similar items. For example, minor modifications of the product title pertaining to colors or measurements majorly impacted the model's output. This phenomenon can negatively affect downstream recommendation or search applications, leading to a sub-optimal user experience. To address this issue, we propose a new framework for consistent text categorization. Our goal is to improve the model's consistency while maintaining its production-level performance. We use a semi-supervised approach for data augmentation and presents two different methods for utilizing unlabeled samples. One method relies directly on existing catalogs, while the other uses a generative model. We compare the pros and cons of each approach and present our experimental results.

==> Chapters/3.related_work.tex <==
\section{Related Work}
{\todo{edit reference mentions}}
The notion of {\it Consistency} in NLP tasks has been studied in several research works~\cite{elazar2021measuring,veitch2021counterfactual,wang2021identifying,jin2020bert,wang2020cat}. A notable study by Elazar et al~\cite{elazar2021measuring} examined the consistency of factual knowledge in Masked Language Models (MLMs) and explored its invariant to paraphrasing using a manually generated dataset. Consistency was also studied as a means of robustness under adversarial attacks. For this task, Di Jin et al.~\cite{jin2020bert} measured the accuracy of the BERT model on manipulated text to evaluate the success of the attack. Another related work was of Tianlu Wang et al.~\cite{wang2020cat}, who trained a generative model to attempt adversarial attacks on a classification model\todo{maybe add more details here}
[Consider remove Arxiv citations-\cite{veitch2021counterfactual} - how to learn a classifier which is robust to spurious correlations (counterfactual invariant).
\cite{wang2021identifying} - We first leverage existing interpretability methods to extract tokens that significantly affect model’s decision process from the input text. We then distinguish “genuine” tokens and “spurious” tokens by analyzing model predictions across multiple corpora and further verify them through knowledge-aware perturbations.] \ariel{Needs rephrasing}




Similarity, numerous approaches for {\it data augmentation} have been explored  for improving various ML tasks, as surveyed in \cite{shorten2021text}. Perhaps the most related to our settings is the work of Kaushik et al.~\cite{kaushik2019learning}, who generated augmented data using human editors, who changed the original samples counterfactually \ariel{did you mean adversarially?}, i.e. they performed small changes so the true label will change, in order to build a robust classifier that doesn't use spurious features. Also, Rizos et al.~\cite{rizos2019augment} generated augmented data to improve hate-speech classification using methods such as replacing words with close words in the embedding space, or using a generative model.
[Consider remove Arxiv citations-
\cite{sennrich2015improving} - using back-translation for augmentation
\cite{ng2020ssmba} - a data augmentation method for generating synthetic training
examples that stay on the underlying data manifold.
\cite{kumar2020data} - text data augmentation using pre-trained Transformer Models. It's include the experiment that we also tried with GPT2
\cite{yang2020generative} - they also use a generative model for text data augmentation]

\subsection{Semi-Supervised Learning}
\cite{xie2020unsupervised} - unsupervised data augmentation for consistency, this paper relate to all of the subjects

\cite{bari2020uxla} - they also have labeled and unlabeled data, and they are doing also self-training and assign pseudo labels, and train a generative model to do augmentation.

\cite{nigam2006semi} - semi-supervised learning of text classification using EM.

\todo{Edit the Appendix to have a similar format to all the  citations and to include all the authors}

\iffalse

\subsection{Data Augmentation in NLP}
\cite{shorten2021text} - a survey for text data augmentation

\cite{sennrich2015improving} - using back-translation for augmentation

\cite{ng2020ssmba} - a data augmentation method for generating synthetic training
examples that stay on the underlying data manifold.

\cite{kaushik2019learning} - they augmented the data using humans that edit the original samples counterfactually, i.e. change them small changes so the true label will change, in order to build robust classifier that don't use spurious features.  

\cite{rizos2019augment} - they use text data augmentation for text classification, using methods such: replacing words with close words in the embedding space, or using a generative model

\cite{kumar2020data} - text data augmentation using pre-trained Transformer Models. It's include the experiment that we also tried with GPT2

\cite{yang2020generative} - they also use a generative model for text data augmentation

\subsection{Consistency in NLP}
\cite{elazar2021measuring} - In this work, we study the consistency of factual knowledge in PLMs, specifically in Masked Language Models (MLMs)—these are PLMs trained with the MLM objective ... We ask: Is the factual information we extract from PLMs invariant to paraphrasing?

\cite{veitch2021counterfactual} - how to learn a classifier which is robust to spurious correlations (counterfactual invariant).

\cite{wang2021identifying} - We first leverage existing interpretability methods to extract tokens that significantly affect model’s decision process from the input text. We then distinguish “genuine” tokens and “spurious” tokens by analyzing model predictions across multiple corpora and further verify them through knowledge-aware perturbations.

\cite{jin2020bert} - they evaluate the robustness of BERT to adversarial attacks. They measure the accuracy of the model on manipulated text to evaluate the success of the attack.

\cite{wang2020cat} - they trained a generative model to do adversarial attack on classification model



\fi
